Instabilities in Multi-Asset and Multi-Agent Market Impact Games

We consider the general problem of a set of agents trading a portfolio of assets in the presence of transient price impact and additional quadratic transaction costs and we study, with analytical and numerical methods, the resulting Nash equilibria. Extending significantly the framework of Schied & Zhang (2019) and Luo & Schied (2020), who considered the single asset case, we prove the existence and uniqueness of the corresponding Nash equilibria for the related mean-variance optimization problem. We then focus our attention on the conditions on the model parameters making the trading profile of the agents at equilibrium, and as a consequence the price trajectory, wildly oscillating and the market unstable. While Schied & Zhang (2019) and Luo & Schied (2020) highlighted the importance of the value of transaction cost in determining the transition between a stable and an unstable phase, we show that also the scaling of market impact with the number of agents J and the number of assets M determines the asymptotic stability (in J and M ) of markets.

==> MIG_multi_agent.tex <==
\section{Instability in market impact games with many agents}\label{sec_multi_agent}

   
  
 

 
   

  
  
%       \begin{figure}[!h]
% \centering


% \caption{Surface plot (left) and the corresponding 
% level curves (right) of $\theta^*$ in function of $M$ and $J$ for fixed $N=300$ and $\gamma=10$.}
% \label{fig_theta*_M_J}
% \end{figure}  

==> hetero_agents.tex <==

\section{Instability and heterogeneity of agents' trading skills}
\label{sec_hetero_agent}
Here we study the case of two agents trading one asset, but, differently from \cite{schied2018market}, we assume that the two agents are different in their trading skills. We consider separately three sources of heterogeneity: different permanent impact, different temporary impact (or trading fees), and different trading speed.


In the first setting, we study the case when the two agents
affect with a different impact the price process. This might correspond to more sophisticated traders who are able to trade more efficiently, for example using better algorithms for posting orders in the market. There is an alternative interpretation, more in line with traditional market microstructure. Permanent impact is considered a measure of the informativeness of trades, thus an agent with a very small permanent impact might be interpreted as a noise trader. In our model the two interpretations are indistinguishable. For analytical convenience, we assume the kernel $G(t)$ is the same for the two agents and we introduce two scaling parameters $\beta_i$ ($i=1,2$) such that the price process dynamic affected by trading becomes\footnote{Note that this is equivalent to saying that the $G(t)$ of the two agents are proportional one to each other, i.e. the two agents differ in the value of $G(0)$.}
\begin{equation}\label{eq_aff_diff_beta}
S_t^{\bm{\xi},\bm{\eta}}=S_t^0-\sum_{k=0}^N G(t-t_k)
(J^{-\beta_1}\xi_k+J^{-\beta_2}\eta_k),
\end{equation}
where $J=2$.  We observe that when two agents have different $\beta$'s this
does not compromise the market stability. Indeed, 
the previous equation can be rewritten as 
 \begin{equation}
     \label{eq_aff_diff_beta_2}
     S_t^{\bm{\xi},\bm{\eta}}=S_t^0-\sum_{k=0}^N G(t-t_k)
(\widetilde{\xi}_k+\widetilde{\eta}_k),
 \end{equation}
 where $\widetilde{\xi}_k,\ \widetilde{\eta}_k$ are the strategies associated with the transformed inventories $\widetilde{X}_0=J^{-\beta_1}X_0$,
  $\widetilde{Y}_0=J^{-\beta_2}Y_0$. Therefore, the Nash equilibrium of 
  equation \ref{eq_aff_diff_beta} is related to the 
  equilibrium of equation \ref{eq_aff_diff_beta_2}, i.e., the are 
  equal up to constants, and in particular the stability is not compromised.
  We just mention that if, for instance, $\beta_1=0$ and $\beta_2=1$, i.e. the impact of the second agent is half the one of the first agent,
  and both agents are Fundamentalist sellers,
  the sophisticated (or uninformed) agent 
  $Y$ has the advantage as if he/she should trade half of his volume.
  %In this case the trader with $\beta_1=0$ has a greater impact than the other player, so we can imagine this trader as a \emph{big} Fundamentalist seller and the counterpart as a \emph{small} one.
  Figure \ref{fig_hetero_betas} exhibits the Nash equilibrium for both traders. As expected, the optimal trading pattern is different for the two traders. More interestingly, the trading profile of the agent with small impact resembles the one of an Arbitrageur (see for comparison Fig. \ref{fig_round_schied}). Thus, from the point of view of the trading profile, an Arbitrageur with zero inventory or a Fundamental trader with small impact behaves in a similar way at equilibrium. Remember that the latter can be seen either as a skilled trader or as a noise trader.   
%It is worth nothing that the shape of the big seller is in some sense asymmetric respect to the typical shape of the standard Schied and Zhang model, see for instance Figure \ref{fig_round_schied}.{\color{red}FC: non mi piace molto come lo ho scritto} 
  Moreover, the expected cost for the $\beta=0$ and $\beta=1$ sellers are equal to $0.6521$ and $0.2582$, respectively. When both agents have $\beta=0$, the costs are equal to 
$0.7975$, thus the reduction of impact of one agent is indeed beneficial to both traders.

             \begin{figure}[!h]
\centering
{\includegraphics[width=0.9\textwidth]{plot_new/hetero_betas.eps}}
\caption{
Nash equilibrium for two Fundamentalist sellers when $\theta=1.5$.
The left (right) figure is referred to the agent with $\beta_1=0$ ($\beta_2=1$).
The trading time grid is an equidistant grid with $26$ points and the decay kernel 
is $G(t)=\exp(-t)$. 
}\label{fig_hetero_betas}
\end{figure}  
% quii

In the second setting, we consider two agents with different temporary impact parameter $\theta$. This might correspond again to the case where one of the two agents has more sophisticated trading strategy or to a market where different class of traders are allowed to pay different fees. This is indeed quite standard for example in ATS where liquidity providers have lower fees than liquidity takers. In particular, we want to test whether only one agent with $\theta$ below threshold is sufficient to destabilize the market or if both agents must have $\theta<\theta^*$.
%In particular we examine the case that when the HFT has a $\theta$ lower than the critical value.
We denote with $\theta_{X}$ and $\theta_Y$ the temporary impact parameter for the two agents. We study the Nash equilibrium by solving numerically the \cite{schied2018market} game in the setting where both agents are Fundamentalist 
 seller with $X_0=Y_0=1$.
 When both agents are above threshold ($\theta^*<\theta_Y<\theta_X=2\theta_Y$, see Figure \ref{fig_theta_HFT_stable}), 
we observe that the more significant difference between the two solutions is in the trading schedule of
low $\theta$ agent, who trades more at the beginning of the trading session. 
%Moreover, by comparing this figure with the case when the two agents have different {\it permanent} impact (Fig. \ref{fig_hetero_betas}), we notice that when one agent has lower $\theta$, her trading profile remains similar to that of a Fundamentalist {\color{blue} where $\beta=0$. "Sono tutti Fund penso che intendevi dire che rimane simile a quello di un Fund con beta zero giusto?}. {\color{blue}In realtà non mi torna molto questo discorso, direi piuttosto che il profilo di trading del Fund rimane abbastanza invariato, simile, se compariamo la Fig 12 con la Figura 2 dove ho Fund e Arbi, così come accade per il caso beta=0 della Figura 11. Che ne pensi?"}
It is interesting to consider the changes in cost. When $\theta=1$ for both agents, the individual cost is $0.7970$. Suppose now that $\theta_Y$ is reduced to $0.5$ (for example because a new type of agent enters the market or because the fee schedule changes for some class of traders). As expected, the expected cost of agent $Y$ is reduced ($0.7317$), but there is a negative effect on the other agent $X$ who sees her cost soar to $0.8286$. Thus, the decrease of $\theta$ for a class of agents impacts negatively the other market participants.

           \begin{figure}[!h]
\centering
{\includegraphics[width=0.9\textwidth]{plot_new/theta_het_fundHFT_stable.eps}}
\caption{Red lines are the Nash equilibrium when both traders have $\theta=1$. Blue lines 
are the solution when $X$ has $\theta=1$ and $Y$ has $\theta=0.5$.
The trading time grid is an equidistant grid with $16$ points and the decay kernel 
is $G(t)=\exp(-t)$. 
%When both agents have homogeneous $\theta=1$, the related expected cost are $0.7970$ for both traders. When $Y$ is a HFT then the expected cost for $X$ raises to $0.8286$, while  it reduces to $0.7317$ for $Y$.
}\label{fig_theta_HFT_stable}
\end{figure}  

When we examine the case when one of the agents has a $\theta_Y$ smaller 
than the critical value $\theta^*=0.25$, 
%{\color{blue} Qui uno potrebbe obiettare dicendo che la figura 13 non mostra un'oscillazione spuria, il fatto è che numericamente non convergo e tutte le soluzioni sono con queste oscillazioni che sono di fatto un artefatto numerico sintomo di instabilità. Infatti se provo a risolvere numericamente SZ model con theta 0 ottengo lo stesso comportamento. Forse conviene non mostrare la figura e scrivere solo il commento che dici? Oppure mettere una nota con quanto ho scritto sopra.}
%As shown in Figure \ref{fig_theta_HFT_unstable}, 
we find numerical evidences that the equilibrium becomes unstable also  for the Fundamentalist agent $X$ for which $\theta_X>\theta^*$. This suggests that in a market with few sophisticated traders with small temporary impact (HFTs) or agents allowed to pay lower fees, the instability 
comes up for all the agents in the market, regardless 
for their own $\theta$s. %\footnote{We remark that we have only examined numerical solutions, which we have truncated after $1000$ iterations, since they tends to oscillate infinite times without reaching equilibrium.}.
%commento su giustificazione teoriche
In other words, market instability is driven by the agent with the smallest $\theta$ and having even few sophisticated traders (in terms of costs or fees) destabilizes the market. 


\iffalse
           \begin{figure}[!h]
\centering
{\includegraphics[width=0.9\textwidth]{plot_new/theta_het_fundHFT_unstable.eps}}
\caption{Red lines are the Nash equilibrium when both traders have $\theta=1$. Blue lines 
are the solution when $X$ has $\theta=1$ and $Y$  has $\theta=0.1$.}\label{fig_theta_HFT_unstable}
\end{figure} 
\fi
The third and last setting assumes that the two traders are different because one of the two is faster than the other. A fast trader could represent, for example, an HFT. In market impact games one has to decides who arrives first in the market at each time step, because the laggard is going to pay the impact of the trade of the leader. In the standard setting, this is decided by a fair Bernoulli trial, which means that on average each trader is the leader half of the times.
We modify this and for each trading time 
$t_k$ the Bernoulli game $\varepsilon_k$ deciding the trading priority, 
is no longer fair, i.e., \[
\varepsilon_k=\begin{cases}
1, \quad \text{with probability } p \\
0, \quad \text{with probability } 1-p
\end{cases}~~~~~~~ p \in [0,1]
\]
where $\varepsilon_k=1$ means that $Y$ places the $k$-th order 
before $X$, so that $X$ has to take into account the impact of $Y$ in her cost. 
%So, $p$ can be interpreted as the trading rate of $Y$ and we assume that the HFT $Y$ is twice as fast the fundamentalist $X$, i.e, $p=2/3$.
Let us denote with 
$\bm{\xi}\ (\bm{\eta})$ the Nash equilibrium for $X$ ($Y$), then
we observe that $\E[C_T (\bm{\xi}|\bm{\eta})]=\E[\frac{1}{2}
\bm{\xi}^T \Gamma_{\theta} \bm{\xi}+\bm{\xi}^T 
\Gamma_p \bm{\eta}]$ and
$\E[C_T (\bm{\eta}|\bm{\xi})]=\E[\frac{1}{2}
\bm{\eta}^T \Gamma_{\theta} \bm{\eta}+\bm{\eta}^T 
\Gamma_{1-p} \bm{\xi}]$, since 
\[
\sum_{k=0}^N \xi_k \left(
p \eta_k+\sum_{m=0}^{k-1} \eta_m G(t_k-t_m)\right)=\bm{\xi}^T 
\Gamma_p \bm{\eta}
 \quad 
\text{ where } (\Gamma_{p})_{i j}=\begin{cases}
\widetilde{\Gamma}_{i j}, \quad i\neq j\\
p\cdot G(0),\quad  i=j
\end{cases}.
\]

 \begin{figure}[t]
\centering
{\includegraphics[width=0.95\textwidth]{plot_new/fundHFT_time.eps}}
\caption{
Nash equilibrium in function of the trading speed $p$ (probability of arriving first on the market) of $Y$.
The red dotted lines are the Nash equilibrium when both traders have the same trading speed, i.e., $p=0.5$. The time grid has $16$ points, $\theta=1$ and $G(t)=\exp(-t)$.}\label{fig_theta_HFT_time}
\end{figure} 

\begin{table}[!h]
\centering
\begin{tabular}{ll|l}
\toprule
$\E[C_T (\bm{\xi}|\bm{\eta})]$ & $\E[C_T (\bm{\eta}|\bm{\xi})]$
& $p$\\
\midrule
0.7970 & 0.7970 & 1/2  \\
0.8173 & 0.7765 & 2/3   \\
0.8274 & 0.7662 & 3/4   \\
0.8333 & 0.7601 & 4/5  \\
0.8568 & 0.7360 & 1    \\
\bottomrule
\end{tabular}
\caption{Expected costs of the two agents $X$ and $Y$ as a function of the trading speed $p$ (probability of arriving first on the market) of $Y$. When $p=1$ the agent
 $Y$ places orders always before of $X$.}\label{tab_ex_cost_p}
\end{table}

Figure \ref{fig_theta_HFT_time} exhibits the Nash equilibrium of the two 
traders for several values of $p$ and Table \ref{tab_ex_cost_p} reports 
the corresponding expected costs. 
We observe that  when $p$ increases, the optimal solution for the HFT $Y$ is to 
liquidate slightly faster in the first period and then 
sell the remaining part of the inventory with a lower intensity, with respect to 
the solution with $p=0.5$, at the end 
of the trading session.
For the slow trader $X$ the behavior is exactly opposite to the one of the fast trader.
However the differences between Nash equilibria for different $p$ are quite small, while
the greatest benefit for the HFT 
is the smaller trading costs  (see Table \ref{tab_ex_cost_p}).

Finally, we ask whether the presence of a fast trader  modifies the critical value of $\theta$ when the instability starts. 
Figure \ref{fig_theta_critic_hft} shows how $\theta^*$
varies as a function of the trading speed $p$
for a games between two Fundamentalist sellers\footnote{We also repeat the same experiment in the presence of an Arbitrageur against a Fundamentalist and we find analogous results.}. Since we compute 
the critical value using a numerical method there are some small oscillations. We observe a small but significant trend of $\theta^*$ as a function of $p$. This result indicates that the presence of an HFT makes the market more prone to oscillations and instabilities. However the effect is relatively small compared to the other possible sources of instabilities studied in the previous sections.
 




        \begin{figure}[!h]
\centering
{\includegraphics[width=0.85\textwidth]{plot_new/theta_critical_hft_fund_average.eps}}
\caption{Numerical estimates
of the critical value $\theta^*$ as a function of the trading speed $p$ (probability of arriving first on the market) of the HFT. We set $N=6$ for the time grid and $G(t)=\exp(-t)$. Both agents are Fundamentalist sellers.}\label{fig_theta_critic_hft}
\end{figure}  


%  Finally, we analyse the game between a Fundamentalist seller $X$ and an Arbitrageur $Y$, when $p\in [0,1].$
%  We recall that when $p$ is close to 1 the Arbitrageur $Y$ places orders almost always before of the Fundamentalist. Figure \ref{fig_theta_HFT_time_arbi}
% exhibits how the shape of the equilibrium varies as a function of $p$. In particular, the solution of the Arbitrageur is very weakly affected by 
% $p$, while for the Fundamentalist 
% we observe that when $p$ is close to 0 the optimal schedule converges to a U-shape form, putting more order at the beginning at the session compared to the standard solution with $p=0.5$. 
% This can be motivated by the fact that when $X$ always places orders before $Y$ basically there is no game\footnote{Since $Y$ is an Arbitrageur there is no competition to liquidate the asset.} for the Fundamentalist and the optimal solution is given by the classical U-shape of the TIM.
% However, it seems to be suggestive that the U-shape is the optimal way to exploit the impact of the Arbitrageur when the Fundamentalist is an ultra-fast trader.
% Vice versa, when $p$ is close to 1, the solution of the Fundamentalist tends to 
% concentrate more order at the end of the trading session similarly to the standard solution with $p=0.5$.
% So, we may conclude that when the Arbitrageur is very fast with respect to the Fundamentalist, the optimal schedule is provided by an asymmetric solution where the seller tends to concentrate more orders when the Arbitrageur puts buy orders.
%           \begin{figure}[!h]
% \centering
% {\includegraphics[width=1\textwidth]{plot_new/fund_arbi_HFT_time_1.eps}}\\
% {\includegraphics[width=1\textwidth]{plot_new/fund_arbi_HFT_time_2.eps}}
% \caption{
% Nash equilibrium as a function of the trading rate $p$ of the Arbitrageur $Y$.
% The red dotted lines are the Nash equilibrium when both traders have the same trading rate, i.e., $p=0.5$. The time grid has $16$ points, $\theta=1$ and $G(t)=\exp(-t)$. {\bf SI POTREBBE RIDURRE LA FIGURA A DUE PANNELLI MOSTRANDO p=0,0.2,0.5,0.8,1}}\label{fig_theta_HFT_time_arbi}
% \end{figure} 

% We conclude by studying the effect of the trading speed of the Arbitrageur on the expected costs, which are reported in Table \ref{tab_ex_cost_p_arbi}. 
% We find that the differences are of the order of $0.001$. However, we have found some possible puzzling results.
% Indeed, surprisingly, from the  point of view of the Arbitrageur
% the optimal trading rate is not $1$, but it is about $0.6-0.7$, which means that the Arbitrageur has to trade with a rate just above the Fundamentalist one. Indeed, when $p=1$ the Arbitrageur cannot exploit the impact of the Fundamentalist order {\bf PERCHE'?}. 
% For the Fundamentalist, the situation seems to be inconsistent, since when $p$ is close to 0 
% his/her expected cost increases and it reaches a minimum for $p=1.$ 
% {\bf Da qui in poi non mi e' chiaro cosa tu voglia dire} This is produced by the impact effect which is exploited by the Fundamentalist when all his/her orders are places after the Arbitrageur\footnote{By looking the optimal shape it is clear that at the end of the session the Fundamentalist earns by the re-balancing of the Arbitrageur.}.
% On the other hand, when $p=0$ the Fundamentalist can not deal with the predatory trading of the Arbitrageur even if it trading rate is higher. This suggests that it is wiser to give another physical interpretation to $p$ rather than to think of it as a trading speed.
%  \begin{table}[!h]
% \centering
% \caption{Expected costs of the Fundamentalist $X$ and Arbitrageur $Y$ as function of the trading speed parameter $p$ of $Y$.}\label{tab_ex_cost_p_arbi}
% \begin{tabular}{ll|l}
% \toprule
% $\E[C_T (\bm{\xi}|\bm{\eta})]$ & $\E[C_T (\bm{\eta}|\bm{\xi})]$
% & $p$\\
% \midrule
% 0.4886 & -0.0336 & 0   \\
% 0.4886 & -0.0341 & 0.1 \\
% 0.4885 & -0.0345 & 0.2 \\
% 0.4883 & -0.0349 & 0.3 \\
% 0.4879 & -0.0352 & 0.4 \\
% 0.4875 & -0.0354 & 0.5 \\
% 0.4869 & -0.0355 & 0.6 \\
% 0.4862 & -0.0355 & 0.7 \\
% 0.4854 & -0.0354 & 0.8 \\
% 0.4844 & -0.0353 & 0.9 \\
% 0.4835 & -0.0351 & 1  \\
% \bottomrule
% \end{tabular}
% \end{table}
%\clearpage


==> old_backup_MIG_multi_agent_old_version.tex <==
\section{Instability in market impact games with many agents}\label{sec_multi_agent}
 We now consider $J>2$ agents trading the same asset (i.e. $M=1$) in order to study 
   how the stability of the market is influenced by an increasing competition. This model represents another important generalization of \cite{schied2018market} which considered only the case $J=2$.
   
The unaffected price process $S_t^0$ is always assumed to be a right continuous martingale in a suitable probability space.
 We denote with 
 $\xi_k^j$ the order flow of agent $j$ at time 
 $t_k$, so that the affected price process is defined as
 \[
 S_t^{\bm{\xi}}:=S_t^0 -\sum_{t_k<t} G(t-t_k) 
 \cdot \sum_{j=1}^J \xi_k^j.
  \]
 and we define $\bm{\xi^j}:=(\xi^j_0,...,\xi^j_{N})^T$. 
  In order to derive the equation for the expected costs of each agent, we need to consider all the possible
   time priorities among the $J$ traders at each time step.  To this end we assume that for each trading time $t_k$ 
 there is a random permutation which determines 
 the time priority, i.e., 
 $\forall k \quad \sigma_k: \{1,2,\ldots,J\}\to \{1,2,\ldots,J\}$, 
 where $\sigma_k(j)$ denotes the position of the
$j$-th agent at time $t_k$.
 Then, let \[\bm{\xi}^{-j}:=(\bm{\xi}^1,\bm{\xi}^2,\ldots,\bm{\xi}^{j-1},\bm{\xi}^{j+1},\ldots,\bm{\xi}^J),\] so if we consider all the possible time 
 priorities among the $J$ agents, we obtain for the execution costs,
\begin{small} 
\[
 C_{\mathbb T}(\bm{\xi}^{j}|\bm{\xi}^{-j})=
 \sum_{k=0}^N \left(
 \frac{G(0)}{2} (\xi_k^j) ^2+G(0)\sum_{i=2}^J
\mathbf{1}_{\{\sigma_k(j)=i\}} 
\sum_{l=1,l\neq j}^J 
\mathbf{1}_{\{\sigma_k(l)<i,\sigma_k(j)=i\}} 
\xi_k^l\xi_k^j-S_{t_k}^{\bm{\xi}}
 \xi_k^j+\theta (\xi_k^j)^2
 \right)+X_0^j S_0^0,
 \] \end{small}
 where $\sum_{k=0}^N \xi_k^j=X_0^j$ denotes the inventory of the $j$-th agent.
  We observe that the trader $j$ pays 
the cost only of the other agents trading before her. Thus at time $t_k$, this cost is given by 
 \[G(0)\sum_{i=2}^J
\mathbf{1}_{\{\sigma_k(j)=i\}} 
\sum_{l=1,l\neq j}^J 
\mathbf{1}_{\{\sigma_k(l)<i,\ \sigma_k(j)=i\}} 
\xi_k^l\xi_k^j,\]
where the indicator function in the first sum selects when the trader $j$ is in position 
$i$ in the arrival queue and the second sum gives the cost of agents trading before 
the $j$-th trader.
Also, since
$\mathbf{1}_{\{\sigma_k(j)=i\}}\cdot \mathbf{1}_{\{\sigma_k(l)<i,\ \sigma_k(j)=i\}} =\mathbf{1}_{\{\sigma_k(l)<i,\ \sigma_k(j)=i\}}$,
the cost to the order $\xi_k^j$  is given by 
  \[G(0)\sum_{i=2}^J
\sum_{l=1,l\neq j}^J 
\mathbf{1}_{\{\sigma_k(l)<i,\ \sigma_k(j)=i\}} 
\xi_k^l\xi_k^j.\]

%  {\bf LA PARTE CHE SEGUE E' DAVVERO NECESSARIA? O ANDREBBE MESSA PRIMA DELLA FACCENDA DELLE INDICATRICI?} The previous definition is motivated by following argument, where we follow a particular selected time priority permutation.
%   We imagine that at time $t_k$ player $1$ decides to place an order and the price moves from $S_{t_k}^\xi$
%  to $S_{t_k^+}^\xi$:
%  \[  
%  S_{t_k^+}^\xi=S_{t_k}^\xi-G(0) \xi_{k,1}.
%  \]
%  However, the order is executed at middle price
%  $(S_{t_k^+}^\xi+S_{t_k}^\xi)/2$ and the 
%  cost for the first agent is 
%  \[
%  -\frac{1}{2} (S_{t_k^+}^\xi+S_{t_k}^\xi)
%  \xi_{k,1}=\frac{G(0)}{2}\xi_{k,1}^2-
%  S_{t_k}^\xi \xi_{k,1}.
%  \]
%   Immediately after the first player, the second agent places an order and moves the price from 
%  $S_{t_k^+}$ to $S_{t_k^{++}}=S_{t_k^+}-G(0)\xi_{k,2}$
%  and his/her cost is given by
%  \[
%  -\frac{1}{2}(S_{t_k^{++}}^\xi
%  +S_{t_k^+}^\xi)\xi_{k,2}=
%  \frac{G(0)}{2}\xi_{k,2}^2+G(0) 
%  \xi_{k,1}\xi_{k,2}-S_{t_k}^\xi \xi_{k,2}.
%  \] 
%  Then, if a third agent places an order we 
%  obtain that his/her cost is
%  \[
%  -\frac{1}{2}(2 S_{t_k^{++}}^\xi
%  -G(0) \xi_{k,3})\xi_{k,3}=
%  \frac{G(0)}{2}\xi_{k,3}^2+G(0) 
%  \xi_{k,1}\xi_{k,3}+G(0) 
%  \xi_{k,2}\xi_{k,3}-S_{t_k}^\xi \xi_{k,3}.
%  \]
%  At the end, the cost of the $J$ agent is given by 
%  \[
%  \frac{G(0)}{2}\xi_{k,J}^2+G(0)
%  \sum_{j=1}^{J-1} \xi_{k,J} \xi_{k,j}-
%  S_{t_k}^\xi \xi_{k,J}.
%  \]
 
 
 In order to compute the expected cost, we need to average over all the permutations of traders' arrival at each time. We prove the following important Lemma useful for the numerical study of 
 equilibrium.

 \begin{lem}\label{lem_cost_multi_agent}
 \[
 \E[C_{\mathbb T}(\bm{\xi}^j|\bm{\xi}^{-j})]=
     \E[\frac{1}{2}(\bm{\xi}^j)^T \Gamma_{\theta} \bm{\xi}^j]+
     \sum_{k=0}^N \xi_k^j \left(
     \sum_{i=2}^J \sum_{l\neq j}
     \frac{(i-1)}{J\cdot (J-1)}
     \xi_k^l+\sum_{m=0}^{k-1} 
     G(t_m -t_k)\sum_{l\neq j}\xi_m^l
     \right).
\]
 \end{lem}
 
 We now analyse numerically the Nash equilibrium emerging from the interaction of different types of agent. Unless otherwise specified, we fix $\theta=10$ and $N=15$. Moreover we introduce a scaling parameter $\beta\geq0$ for the kernel function when $J$ increases, i.e.,
 $G(t)=J^{-\beta}e^{-t}$. The case when $\beta=0$ corresponds to the 
 additive case, while for $\beta=1$ the total instantaneous impact does not depend on the number of agents.
 Hence, when $\beta=1$ the aggregate impact of all the agents is independent from $J$ and we want to test whether the trading patterns are also independent from it. Recent empirical evidences (\cite{coimpact}) show that market impact depends on the aggregate net order flow of the optimal executions simultaneously present, without individually distinguishing them.
 
 \begin{sidewaysfigure}
\centering
{\includegraphics[width=1\textwidth]{plot_new/fund_multi_agent_conrescaling.eps}}
\caption{Optimal solution of a fundamental seller for different number $J$ of agents and when the scaling parameter $\beta$ is set to $0,1/2,1$. The time grid contains $16$ points.}\label{fig_fund_multi_agent}
\end{sidewaysfigure} 
 
 To this end, we first study an homogeneous  market with $J$ identical Fundamentalist sellers with the same initial inventory. In Figure \ref{fig_fund_multi_agent} we report the Nash equilibria
for the agents when $\beta=0,1/2,1$ and 
for different values of $J$.
We remark
that for each $\beta$ the initial inventory $X_0^j$, for all agent $j$, is rescaled by $J^{-\beta}$, and then, for improve readability, 
the displayed solutions are normalized such that the sum of 
orders is equal to $1$.




  When the competition in the market increases, regardless of $\beta$, the optimal solution tends to place more orders
at the beginning of the trading sessions, instead of waiting the last trading time. This synchronized trading of all the agents at the beginning of the trading period, as resulting from the Nash equilibrium, could be at the origin of the market instability. 
 On the other hand, when $\beta$ increases the equilibrium seems to be approximated by a flat straight line with a constant
trading volume over time. In any case, it is important to notice that when $\beta=1$ the Nash equilibrium is {\it not} independent from the number of agents $J$. Thus, for example, the equilibrium of $J=2$ agents is not the same as the equilibrium of $J=4$ agents with half the impact and half the initial inventory\footnote{This analysis assumes that the initial inventory is the same for the agents. In Appendix \ref{app_shape_analysis}
we explore the case when 
this assumption is relaxed.}. 



%              \begin{figure}[!h]
% \centering
% {\includegraphics[width=1\textwidth]{plot_new/cost_multi_agents.eps}}
% \caption{Expected cost of a fundamentalist in a competitive  market when the scaling parameter $\beta$ is set to $0,1/2,1$. All agents are identical Fundamentalist sellers, $\theta=10$ and the time grid contains $16$ points.}\label{fig_cost_multi_agent}
% \end{figure} 



              \begin{figure}
\centering
{\includegraphics[width=.8\textwidth]{plot_new/theta_critical_multi_agent.eps}}
\caption{Numerical estimates of the critical value of $\theta$ as a function of the number of agents when the time grid is fixed with $7$ points for some scaling parameters. All agents are identical Fundamentalist sellers.}\label{fig_theta_multi_agents}
\end{figure} 
 
 
We now consider, in the same setting as above, how the stability of the market depends on the number of agents and on the scaling parameter $\beta$. Specifically, we compute numerically the critical value of $\theta$ after which
   the market is not stable.
We choose a time grid equal to $N=6$ and we study the three cases when $\beta=0,1/2, 1$
by increasing the number of agents.
%, where all considered agents are fundamental seller.
   We find that the increase of competition of the market, i.e. a larger number of agents competing for the same objective,   deteriorates its stability increasing $\theta^*$ (see  Figure \ref{fig_theta_multi_agents}). For $\beta=0$ the points lie approximately on a line and the addition of an agent increases $\theta^*$ by approximately $0.4$.
 On the other hand,
the instability seems to be relaxed when the scaling parameter increases, where the relation with $J$ becomes flatter.  Notice however that when $\beta=1$, i.e. the total impact of agents becomes approximately independent from $J$, $\theta^*\to 0.4$ when $J$ increases, and this asymptotic value is larger than the one for two agents which is $\theta^*=0.25$. We conclude that the increase of the competition in a market may deteriorates 
its stability and, less surprisingly, it increases the expected costs of a strategy.
 


% We then, fix $\theta=10$ in order to consider only stable equilibria and
% we show how the expected costs of a fundamentalist seller varies
% when he/she is in competition with other sellers (see Figure \ref{fig_cost_multi_agent}). We observe that the expected cost
% increases linearly with the number of agents.
% We also choose a scaling parameter $\beta$ equal to $1/2$ and $1$ 
% together with the standard case. We observe when the impact of the 
% single agents decreases with the population size, the expected cost tends
% to be flat {\bf A ME SEMBRA CHE RESTI LINEARE}.





%For $J>2$ we study two situations: i) when all the sellers change their inventories by the same amount of shares and ii) when there is a seller who trades against a volume which is greater than his inventory. As for $J=2$ the shape of the Nash equilibrium is invariant to the inventories of agents if they are all equal also when $J>2$. Figure\ref{fig_agents_V1_05} exhibits the Nash equilibrium for 4 seller with inventories equal to 1 and 0.5. Clearly, the shape of the solution is the same for both cases, but the differences is due a scaling which is the total volume traded by agents as for the two agents case.



 
 
 Now we consider the cases when the agent are of different types. In particular, we focus on the role of an Arbitrageur when two other agents are either identical or of opposite type.  

First, we consider the case of two identical Fundamentalist sellers and one Arbitrageur ($J=3$) and we fix 
$\theta=1.5$. Figure \ref{fig_3_agent} (left) displays the equilibrium solution for $\beta=0$, to be compared with the two agent case of Fig. \ref{fig_round_schied}.
While the trading pattern of the Arbitrageur is qualitatively similar to the one of the two agent case, the Fundamentalists trade significantly less toward the end of the day. This is likely due to the fact that it might be costly to trade for one Fundamentalist given the presence of the other. The expected costs for the two Fundamentalists is equal to  $0.9125$ and $-0.0885$ for the Arbitrageur.

              \begin{figure}
\centering
% {\includegraphics[width=0.8\textwidth]{plot_new/multi_agent_sell_buy_arbi.eps}}\\
% {\includegraphics[width=0.8\textwidth]{plot_new/multi_agent_sell_buy_arbi2.eps}}
\centering
{\includegraphics[width=0.45\textwidth]{plot_new/multi_agent_sellers_arbi.eps}}
{\includegraphics[width=0.45\textwidth]{plot_new/multi_agent_sell_buy_arbi_box.eps}}
\caption{Blue and red lines are the Nash equilibrium for the Fundamentalist traders. The yellow line refers to the equilibrium of the Arbitrageur. The scaling parameter $\beta$ is set to $0$.}\label{fig_3_agent}
\end{figure} 

We then consider the case of a Fundamentalist buyer, a Fundamentalist seller and an Arbitrageur in order to see whether this last agent is able to exploit, as a sort of market maker, his/her position. Figure \ref{fig_3_agent} (right) shows the Nash equilibrium for this case. It is clear that the Arbitrageur barely trades and the expected costs are $0.13$ and $-3.98\cdot 10^{-07}$ for the two Fundamentalists and the Arbitrageur, respectively. This indicates that the two Fundamentalists are able to reduce significantly their costs with respect to the previous case, increasing their protection against predatory trading strategies and that the Arbitrageur is not able to act as a market maker.
    On the other hand, we observe (see the inset of Fig. \ref{fig_3_agent}) that the solution for the 
    Arbitrageur starts to exhibit some oscillations of purchase and sale,
    although
    his/her orders remains of negligible size with respect to that of Fundamentalists.
    





 



%commento su i due plot  con tutti stesso inventario
%commento su i plot con 0.5 vs 7/6 e 
%  1/10 contro 13/10 e paragone con S&Z quando diffferenza tende -X_2^0 no U-shape

%\clearpage

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


